Regret Analysis of a Markov Policy Gradient Algorithm for Multi-arm Bandits

We consider a policy gradient algorithm applied to a finite-arm bandit problem with Bernoulli rewards. We allow learning rates to depend on the current state of the algorithm, rather than use a deterministic time-decreasing learning rate. The state of the algorithm forms a Markov chain on the probability simplex. We apply Foster-Lyapunov techniques to analyse the stability of this Markov chain. We prove that if learning rates are well chosen then the policy gradient algorithm is a transient Markov chain and the state of the chain converges on the optimal arm with logarithmic or poly-logarithmic regret.

==> THEOREM_2.tex <==

\section{Proof of Theorem \ref{2nd_theorem}.}
\label{AppendixB}


The proof of Theorem \ref{2nd_theorem} follows the same structure Theorem \ref{main_theorem}: we bound the expected recurrence time to the set $\{ p_{a^\star} > 1/2 \}$; we study the embedded chain $\hat q(s)$, which follows $q_{a^\star}$when $q_{a^\star} < 1/2 $ holds; we analyze the transient behavior of $(p_a(t) : a\in \mathcal A)$ and show this distribution concentrates on the correct arm; and finally, we prove Theorem \ref{2nd_theorem}.

Most steps of the argument are identical to Theorem \ref{main_theorem}. We point the reader to the appropriate parts in the proof of Theorem \ref{main_theorem}, when they are used in Theorem \ref{2nd_theorem}. The results that change are Lemma  \ref{upperbound}, Proposition \ref{first_lemma}  and Proposition \ref{LemExpectq} which are replaced by Lemma \ref{upperbound_2}, Proposition \ref{2nd_lemma} and Proposition \ref{LemExpectq_2}. We prove these below, and restate other results with an identical proof to prior results.

\subsection{Recurrence Times.}
\label{app:recurrence}

First, before we get going, notice the heuristic argument in the introduction analyses the differential equation $\dot p = -\alpha \Delta p^2$ which implies $1/p(T) - 1/p(0) = \alpha \Delta T$. Thus there we used $1/p(t)$ as a Lyapunov function.
In this section, the analogous differential equation is
\[
\dot p  
=
\frac{\beta\Delta p^2}{1-\log p}
\quad
\text{ which implies }
\quad 
T\beta \Delta 
=
\int_{p(T)}^{p(0)}
\frac{1-\log p}{p^2}{\rm d} p 
=
\frac{1}{p(T)}
\log \frac{1}{p(T)}
-
\frac{1}{p(0)}
\log 
\frac{1}{p(0)}\, .
\]
So we now use $\frac{1}{p(t)}\log \frac{1}{p(t)} $ as a Lyapunov function. The following is a deterministic version of the aforementioned differential equation.

We replace Lemma \ref{upperbound} with the following:

\begin{lemma}
	\label{upperbound_2}
	If $\bar q(t)$ is a sequence of real numbers belonging to the interval $(0,1)$ such that 
	\begin{equation}\label{qbounds}
	\bar q (t+1)
	-
	\bar q (t)
	\leq 
	-
	\frac{\eta \bar q(t)^2}{
		1-\log ( \theta \bar q(t) )
	}	
	\end{equation}
	for $\theta \bar q(0) \leq 1$, 
	then, for $\eta T/ \theta \geq e$,
	\[
	\bar q (T) 
	\leq
	\frac{1 }{\eta T}
	\log \Big(
	\frac{\eta T}{ \theta } 
	\Big) \, .
	\]
\end{lemma}
 \Beginproof
	Firstly it is clear that $\bar q(t)$ is a decreasing sequence. Notice that the inequality \eqref{qbounds} rearranges to give 
	\[
	\frac{1-\log(\bar q(t) \theta)}{\bar q(t)^2}
	\big[ 
	\bar q(t) 
	-
	\bar q(t+1)
	\big]
	\geq \eta \, .
	\]
	Summing we see that 
	\begin{equation}
	\label{RS:sum}
	\sum_{t=0}^{T-1}
	\frac{1-\log(\bar q(t) \theta)}{\bar q(t)^2}
	\big[ 
	\bar q(t) 
	-
	\bar q(t+1)
	\big]
	\geq
	\eta T \, .	
	\end{equation}
	We could interpret this as a Riemann-Stieltjes approximation to the integral
	\[
	\int_{\bar q(T)}^{\bar q(0)}
	\frac{1-\log (\theta \bar q)}{\bar q^2}
	d \bar q
	=
	\left[
	\frac{\log (\theta \bar q) }{\bar q}
	\right]_{\bar q(T)}^{\bar q(0)}
	=
	\frac{1}{\bar q(T)}
	\log 
	\left(
	\frac{1}{\theta \bar q(T)}\right)
	-
	\frac{1}{\bar q(0)}
	\log \left(
	\frac{1}{\theta \bar q(0)} \right)
	\]
	Since the function $\bar q \mapsto 	\frac{1-\log (\theta \bar q)}{\bar q^2}$ is decreasing on $(0,1/\theta)$ the integral above upperbounds the sum in \eqref{RS:sum}, we have that 
	\[
	\frac{1}{\bar q(T)}
	\log\left( \frac{1}{\theta \bar q(T)}\right)
	-
	\frac{1}{\bar q(0)}
	\log \left(\frac{1}{\theta \bar q (0) }\right)
	\geq 
	\eta T\, .
	\]
	If we let $z(T) = \log \frac{1}{\theta \bar q(T)}$ then we have that
	\begin{equation}\label{z_time}
	z(T) e^{z(T)} 
	\geq 
	\frac{1}{\theta \bar q(0)}
	\log \left( \frac{1}{ \theta\bar q(0)}\right)
	+
	\frac{\eta T}{\theta}
	\geq 
	\frac{\eta T}{\theta} 
	\end{equation}
	The inverse of the increasing function $z\mapsto y := ze^z$ is Lambert's $W$-function for which it is known that 
	\[
	W(y) \geq \log y - \log\log y  = \log \Big( \frac{y}{\log y} \Big) 
	\]
	for $y \geq e$.\footnote{To verify this inequality, notice $z = \log ( y/\log y)$ is such that $ze^z \leq y$ for $y \geq e$. So $W(y)\geq \log (y/\log y)$ .}
	Thus applying the above bound to \eqref{z_time} with $y= \eta T / \theta$ gives
	\begin{equation*}
	\log \frac{1}{\theta \bar q(T)}
	=z(T)
	\geq 
	W\Big( 
	\frac{\eta T}{\theta} 
	\Big)
	\geq 
	\log \left(
	\frac{\frac{\eta T}{\theta} }{\log \Big(\frac{\eta T}{\theta}\Big) }
	\right)
	\end{equation*}
	which implies 
	\[
	\bar q (T) 
	\leq
	\frac{1}{\eta T}
	\log \Big(
	\frac{\eta T}{ \theta} 
	\Big) \, .
	\]
%	For the final inequality note that 
%	\[
%	\frac{1}{\eta T}
%	\log \Big(
%	\frac{\eta T}{ \theta} 
%	\Big)
%	=
%	\frac{1}{\eta T}
%	\log (
%	{\eta T}
%	)
%	-
%	\frac{1}{\eta T}
%	\log \theta
%	\leq 
%	\frac{\theta}{\eta T}
%	\log (
%	{\eta T}
%	)
%	+
%	\frac{e^{-1}}{\eta T}
%	\]
%	where the inequality holds because $\bar q(0)\leq 1$ and because the function $z\mapsto z\log z$ is minimized at $z=e^{-1}$.
  \Endproof

The statement of Proposition \ref{first_lemma} remains much the same but the proof differs.

\begin{proposition}\label{2nd_lemma}
	For $\alpha(p) = \frac{\beta}{1-\log p}$,
	%\begin{equation}\label{lem:alpha}
	%\alpha < \frac{\Delta}{r^{\star} - \Delta}	
	%\end{equation}
	there exists a positive constant $\hat x$ such that 
	\[
	\sup_{\bm p \in E(\hat x)}
	\mathbb E \big[ \tau(\hat x) 
	|
	\bm p (0) = \bm p
	\big]
	< \infty \, .
	\]
\end{proposition}
\Beginproof
	We will show that 
	\[
	\frac{1}{p_{a^\star}(t)}
	\log \frac{1}{p_{a^\star}(t) }
	-
	ct
	\]
	is a supermartingale for some $c>0$. 
	
	Note that (as in the proof of Proposition \ref{first_lemma}) if we let $x(t) = p_{a^\star}(t)^{-1}$ then, a short calculation gives, 
	\[
	x(t+1) 
	=
	\begin{cases}
	x(t) 
	-
	\frac{\alpha}{1+\alpha}
	x(t)
	&
	\text{ w.p. } 
	\frac{r^\star}{x(t)}\, ,
	\\
	x(t)
	\cdot  
	\frac{	
		p_\star (t) x (t)
	}{
		p_\star (t) x(t) - \alpha  
	}
	& \text{ w.p. } p_{\star}(t) r_{\star}(t)\, ,
	\\
	x(t) & \text{ otherwise.}
	\end{cases}
	\]
	Where $r_{\star}(t)$ and $p_{\star}(t)$ are the reward and probability of playing the leading arm at time $t$.
	We apply the shorthand 
	$\alpha = \alpha(x(t)^{-1})$, $x=x(t)$, $r_{\star}=r_{\star}(t)$ and $p_{\star}=p_{\star}(t)$. We have that
	\begin{subequations}
		\begin{align}
		& \mathbb E 
		\Big[
		x(t+1) \log x(t+1) 
		\big| H(t)
		\Big]
		- x(t) \log x(t)
		\notag
		\\
		=
		&
		\frac{r^\star}{x}
		\Big[
		\frac{x}{1+\alpha}
		\log \frac{x}{1+\alpha}
		-x\log x
		\Big]
		+
		p_{\star} r_{\star} 
		\Big[
		x \cdot 
		\frac{p_{\star} x}{p_{\star} x - \alpha}
		\cdot 
		\log \left(
		x \cdot 
		\frac{p_{\star} x}{p_{\star} x - \alpha}
		\right)
		- 
		x \log x
		\Big]
		\notag
		\\
		=
		& 
		-\frac{\alpha}{1+\alpha}
		r^\star \log x
		-
		\frac{r^\star}{1+\alpha }
		\log (1+\alpha)
		\label{term1}
		\\
		&
		+
		p_\star r_\star \cdot 
		\frac{\alpha}{p_{\star} x - \alpha }
		\cdot x \log x 
		\label{term2}
		\\
		&
		+
		p_\star r_\star x 
		\cdot 
		\frac{p_\star x}{p_\star x - \alpha}
		\cdot 
		\log \Big(
		\frac{p_\star x}{p_\star x - \alpha}\Big)\, .
		\label{term3}
		\end{align}
	\end{subequations}
	We upperbound each of the three terms above.
	
	For term \eqref{term1}, we use the following inequalities
	\[
	\frac{1}{1+\alpha} \geq (1-\alpha)
	\quad
	\text{and}
	\quad 
	-
	\frac{r^\star}{1+\alpha }
	\log (1+\alpha)
	\leq 0\, .
	\]
	and
	\[
	\alpha \log x = \beta - \frac{\beta}{1+\log x}
	\quad\text{and}\quad 
	\alpha^2 \log x \
	\leq \frac{\beta}{1+\log x} \, .
	\]
	\begin{subequations}
		These give the following bound for \eqref{term1}
		\begin{equation}
		\label{term1-done}
		-\frac{\alpha}{1+\alpha}
		r^\star \log x
		-
		\frac{r^\star}{1+\alpha }
		\log (1+\alpha)
		\leq 
		- r^\star \alpha \log x
		+
		r^\star \alpha^2 \log x
		\leq 
		-  \beta r^\star 
		+ \frac{2\beta}{1+\log x}\, .	
		\end{equation}
		
		For the term \eqref{term2}, we use the inequalities
		\[
		\alpha \log x
		\leq 
		\beta
		\qquad
		\text{and}
		\qquad 
		\frac{\alpha}{
			p_\star x -\alpha}
		\leq 
		\frac{N\beta}{x(1+\log x) - N\beta }
		\]
		The second inequality above holds by substituting the value of $\alpha$ and noting that $p_\star \geq \frac{1}{N}$. These applied to the term \eqref{term2} give
		\begin{align}
		p_\star r_\star \cdot 
		\frac{\alpha}{p_{\star} x - \alpha }
		\cdot x \log x 
		&
		=
		r_\star \cdot
		\frac{
			p_\star x }{
			p_{\star} x -\alpha 
		}
		\cdot 
		\alpha \log x
		\notag 
		\\
		&
		=
		r_\star  
		\cdot \alpha \log x
		+ r_\star
		\cdot 
		\alpha \log x
		\cdot 
		\frac{\alpha}{p_{\star} x - \alpha }
		\notag 
		\\
		&
		\leq 
		\beta r_\star  
		+
		\beta
		\frac{N\beta}{x(1+\log x) - N\beta }
		\label{term2-done}
		\end{align}
		
		For the term \eqref{term3}, we have that 
		\begin{align*}
		p_\star r_\star x 
		\cdot 
		\frac{p_\star x}{p_\star x - \alpha}
		\cdot 
		\log \Big(
		\frac{p_\star x}{p_\star x - \alpha}\Big)	
		=
		- p_\star r_\star x
		\cdot 
		\frac{
			\log \Big( 1- \frac{\alpha}{p_\star x}\Big)
		}{1- \frac{\alpha}{p_\star x}}
		\end{align*}
		We now take a few moments to show that $-\log (1-z)/(1-z) \leq z+ 4z^2$ for $0\leq z\leq \frac{1}{3}$: We require
		\[
		-\log (1-z) \leq (1-z) ( z+4z^2) = z+ 3z^2-4z^3
		\]
		Both side agree at $z=0$ and differentiating gives a sufficient condition: that for $0 \leq z \leq 1/3$
		\[
		\frac{1}{1-z} 
		\leq 1+6 z - 12 z^2,
		\quad 
		\text{or equivalently}
		\quad 
		0 \leq 5 - 18z + 12z^2.
		\]
		Inspecting the quadratic term on the right hand side. It is positive for $z=1/3$ negative for $z=1$ and positive for $z=2$. So the required inequality holds and thus we have as required that
		\[
		- \frac{\log (1-z) }{1-z}
		\leq z + 4 z^2
		\]
		for $0\leq z \leq 1/3$. Applying this to \eqref{term3} gives
		\begin{align}
		p_\star r_\star x 
		\cdot 
		\frac{p_\star x}{p_\star x - \alpha}
		\cdot 
		\log \Big(
		\frac{p_\star x}{p_\star x - \alpha}\Big)	
		&
		=
		- p_\star r_\star x
		\cdot 
		\frac{
			\log \Big( 1- \frac{\alpha}{p_\star x}\Big)
		}{1- \frac{\alpha}{p_\star x}}
		\notag
		\\
		&
		\leq 
		p_\star r_\star x \cdot 
		\left[
		\frac{\alpha}{p_\star x}
		+4
		\frac{\alpha^2}{p^2_\star x^2}
		\right]
		\leq \frac{\beta}{1+\log x} 
		+
		\frac{2N\beta^2}{x (1+\log x)^2} 
		\label{term3-done}
		\end{align}
		where the first inequality holds
		for all $x$ such that $\frac{\alpha}{p_\star x} \leq \frac{1}{3} $ and in the second inequality we recall the $p_\star \geq \frac{1}{N}$.
	\end{subequations}
	
	Applying bounds 
	\eqref{term1-done}, 
	\eqref{term2-done}
	and 
	\eqref{term3-done}
	to 
	\eqref{term1}, \eqref{term2} and
	\eqref{term3} gives that
	\begin{align*}
	& \mathbb E 
	\Big[
	x(t+1) \log x(t+1) 
	\big| H(t)
	\Big]
	- x(t) \log x(t)
	\notag
	\\
	\leq &
	-  \beta r^\star 
	+
	\beta r_\star  
	+ \frac{2\beta}{1+\log x}
	+
	\beta
	\frac{N\beta}{x(1+\log x) - N\beta }
	+
	\frac{\beta}{1+\log x} 
	+
	\frac{2N\beta^2}{x (1+\log x)^2} 
	\\
	\leq 
	&
	- \beta \Delta
	+
	O\Big(\frac{1}{1+\log x} \Big)\, .
	\end{align*}
	Thus for $\epsilon \in (0,1)$ there exists an $\hat x$ such that for all $x \geq \hat x$ we have that 
	\[
	\mathbb E 
	\Big[
	x(t+1) \log x(t+1) 
	\big| H(t)
	\Big]
	-
	x\log x
	\leq - \beta \Delta (1-\epsilon) =: -c
	\]
	The remainder of the proof is identical to the argument in Proposition \ref{first_lemma} : 
	Since $x(\tau(\hat x) \wedge t)$ is positive and by the Optional Stopping Theorem,
	\begin{equation}
	\label{xbound}
	- \mathbb E [x(1)\log x(1) ] 
	\leq 
	\mathbb E [ x(\tau(\hat x) \wedge t) \log x(\tau(\hat x) \wedge t)]
	-
	\mathbb E [ x(1)\log x(1) ] 
	\leq - c \mathbb E [(\tau(\hat x) \wedge t) -1 ] \, .	
	\end{equation}
	%[Above, $x\wedge y:= \min \{ x,y\}$.]
	Note since, at time zero, $x(0) \leq \hat x $ and $x(1) \geq \hat x $, the most $p_{a^\star}(0)$ can decrease by over the next time step is a factor of $(1-\alpha)$. So
	\[
	x(1) \log x(1)= \frac{1}{p_{a^\star} (1) } \log  \frac{1}{p_{a^\star} (1) } \leq \frac{\hat x}{1-\alpha}
	\log 
	\frac{\hat x}{1-\alpha}\, .
	\]
	Applying the above bound and the Monotone Convergence Theorem to \eqref{xbound} gives
	\[
	\mathbb E [ \tau(\hat x) ]
	=
	\lim_{t\rightarrow\infty}
	\mathbb E [ x(\tau(\hat x) \wedge t)]
	\leq c +\frac{\hat x}{1-\alpha}
	\log 
	\frac{\hat x}{1-\alpha} ,
	\]
	as required.
\Endproof


With Lemma \ref{upperbound_2} and Proposition \ref{2nd_lemma} replacing Lemma \ref{upperbound} and Proposition \ref{first_lemma}, we can reprove Corollary \ref{prop1}. The proof of one supporting lemmas for Corollary \ref{prop1} changes slightly.
We restate the corollary here, and refer the reader to Appendix \ref{corol5} for its proof. 
\begin{corollary}
	\label{prop1_again}
	\[
	\sup_{\bm p \in E(2)}
	\mathbb E[ \tau  |
	\bm p(0)=\bm p] < \infty \, .
	\]
\end{corollary}

\subsection{An Embedded Chain.}
\label{app:embedding}
The embedded chain $(\hat q(s) : s\in \mathbb Z_+)$ is defined in an identical manner to Section \ref{sec:embedding}. 
Proposition \ref{LemExpectq} below is very similar to to Proposition \ref{LemExpectq_2}, with the main modification to its statement being to the bound in part c). For this we require the following technical lemma about the learning rate $\gamma(p) [=p^2 \alpha(p)]$.

\begin{lemma}\label{gamma_bound}
	The step size function 
	\[
	\gamma(p)= \frac{p^2}{1-\log p}
	\]
	is increasing and convex on the interval $p\in (0,1)$.
\end{lemma}
\Beginproof
We can verify this by differentiating $\gamma(p)$. Differentiating once
\[
\gamma'(p) 
=
\frac{2p}{1-\log p} 
+
\frac{p}{(1-\log p)^2}
\geq 0
\]
Differentiating once more gives
\[
\gamma''(p) = \frac{2}{1-\log p} + \frac{3}{(1-\log p)^2}
+
\frac{2}{(1-\log p)^3}
\geq 0\,.
\]
Thus $\gamma(p)$ is increasing and convex for $p\in (0,1]$.
\Endproof
The following result replaces Proposition \ref{LemExpectq}.

\begin{proposition}
	\label{LemExpectq_2}
	For the process $(\hat q(s) : s\in \mathbb Z_+)$ \\
	a)
	\begin{equation}\label{qIneq}
	\mathbb E [ \hat q(s+1) | \hat H(s)  ]
	-
	\hat q(s) 
	\leq 
	-\Delta \beta
	\frac{1}{N}
	\frac{\hat q(s)^2}{
		1-\log (\frac{\hat q(s)}{N})} \, .
	\end{equation}
	and, thus, it is a positive supermartingale.\\
	b) With probability $1$,
	\[
	\hat q(s) \xrightarrow[s\rightarrow \infty]{} 0\, .
	\]
	c)  For $s\beta \Delta \geq e$,
	\begin{equation}\label{qTime2}
	\mathbb E [ \hat q (s) ]
	\leq 
	\frac{N}{s \beta \Delta} \log (s \beta \Delta)  .	
	\end{equation}
\end{proposition}
\Beginproof
	a)  By the identical argument used to derive \eqref{q4} in Proposition \ref{LemExpectq}, we have that
	\begin{align}
	\mathbb E [ \hat q(s+1) | \hat H(s)  ]
	-
	\hat q(s) 
	&
	\leq 
	- \Delta\!\!\! \sum_{a: a\neq a^\star} 
	\alpha (p_a(t_s) )
	p_a(t_s)^2
	=
	- \Delta\!\!\! \sum_{a: a\neq a^\star} 
	\beta
	\frac{p_a(t_s)^2}{1-\log p_a(t_s)} \, .
	\label{q4_2}
	\end{align}
	%We now bound the expectation in \eqref{q4} by twice applying 
	By Lemma \ref{gamma_bound} the terms in the righthand side of \eqref{q4_2} are convex. So
	by Jensen's inequality:
	\[
	\frac{1}{N-1}
	\sum_{a: a\neq a^\star} 
	\frac{p_a^2}{1-\log p_a}
	\geq 
	\frac{
		\left( 
		\sum_{a\neq a^\star} 
		\frac{p_a }{N-1}
		\right)^2
	}{
		1-\log \left(
		\sum_{a\neq a^\star}
		\frac{p_a }{N-1}
		\right)
	}
	=
	\frac{1}{(N-1)^2}
	\frac{\hat q^2}{
		1-\log (\frac{\hat q}{N-1} ) }\, .
	\]
	Applying this to \eqref{q4_2} gives
	\[
	\mathbb E [ \hat q(s+1) | \hat H(s)  ]
	-
	\hat q(s) 
	\leq 
	-\Delta \beta
	\frac{1}{(N-1)}
	\frac{\hat q^2}{
		1-\log (\frac{\hat q}{N-1})} 
	\leq 
	-\Delta \beta
	\frac{1}{N}
	\frac{\hat q^2}{
		1-\log (\frac{\hat q}{N})} \, .
	\]
	Thus \eqref{qIneq} holds as required.
	
	b) The proof of this part is identical to the argument in Proposition \ref{LemExpectq}. So we do not repeat it here.
	
	c) Taking expectations on both sides of \eqref{qIneq} and applying Jensen's Inequality again,
	\begin{align*}
	\mathbb E [ \hat q (s+1) ]
	-
	\mathbb E[\hat q (s) ] 
	&
	\leq 
	-\beta N \Delta 
	\mathbb E 
	\left[
	\frac{ (\frac{\hat q(s)}{N})^2}{
		1-\log (\frac{\hat q(s)}{N})} 
	\right]
	\\
	&
	\leq 
	-\beta N \Delta 
	\frac{
		\left(\frac{\mathbb E[\hat q(s)]}{N}\right)^2 }{
		1
		-
		\log \left(
		\frac{\mathbb E[\hat q(s)]}{N}
		\right)
	}
	=
	-\frac{
		\beta \Delta}{N}
	\frac{\mathbb E[ \hat q (s) ]^2
	}{
		1-
		\log( \frac{1}{N} \mathbb E [\hat q(s)])
	}	\, .
	\end{align*}
	
	
	Thus applying Lemma \ref{upperbound_2} (with $\eta = \beta \Delta /N$ and $\theta = 1/N$), we have that 
	\[
	\mathbb E [\hat q(s) ]
	\leq 
	\frac{N  }{\beta \Delta s}
	\log \Big(
	\frac{\beta\Delta s}{ N \frac{1}{N}} 
	\Big) 
	=\frac{N}{s \beta \Delta} \log (s \beta \Delta) \, .
	\]
\Endproof

\subsection{Transience.}
\label{app:transience}

%Lemma \ref{recurrence_prob_lemma} and
Proposition \ref{trans_prob_prop} can be repeated without change:


%\begin{lemma}\label{recurrence_prob_lemma_2}
%	If $q_{a^\star}(0) \leq  \frac{1}{2}$ then, there exists a constant $\rho < 1$ such that 
%	\begin{equation}\label{hit_prob_1}
%	\mathbb P ( \sigma^{(1)} < \infty ) < \rho\, .		
%	\end{equation}
%Moreover
%\begin{equation}\label{hit_prob_2}
%		\mathbb P ( \sigma^{(k)} < \infty | \sigma^{(k-1)} <\infty)
%	< \rho \, .
%\end{equation}
%\end{lemma}

%The proof Lemma \ref{recurrence_prob_lemma}, which is given in Section \ref{sec:recurrence_prob_lemma}, uses the fact that, by Proposition \ref{LemExpectq}, $q_{a^\star}(t\wedge \sigma^{(1)})$ is a positive supermartingale which, unless stopped, goes to zero. We can use the Optional Stopping Theorem to upper-bound the maximum of this process.
%whose limit is zero on the event $\sigma^{(1)} =\infty$. We can
%and is $\sigma^{(1)} = \infty$ then $q_{a^\star}(t) = \hat q (t) \rightarrow 0$ as $t\rightarrow\infty$.

\begin{proposition}
	\label{trans_prob_prop_2}
	a) If $q_{a^\star}(0) \leq  \frac{1}{2}$ then, there exists a constant $\rho < 1$ such that 
	\begin{equation}\label{hit_prob_1}
	\mathbb P ( \sigma^{(1)} < \infty ) < \rho\, .		
	\end{equation}
	Moreover
	\begin{equation}\label{hit_prob_2}
	\mathbb P ( \sigma^{(k)} < \infty | \sigma^{(k-1)} <\infty)
	< \rho \, .
	\end{equation}
	b) 
	\[
	\sum_{t=0}^\infty
	\mathbb P 
	\Big(
	q_{a^\star} (t) \geq \frac{1}{2}
	\Big)	
	< \infty \, .
	\]
	c) With probability $1$,
	\[
	q_{a^\star}(t) \xrightarrow[t\rightarrow \infty ]{}
	0.
	\]
\end{proposition}

\noindent The proof of Proposition \ref{trans_prob_prop_2} is identical to the proof of Proposition \ref{trans_prob_prop}, with the only change being which results are applied: we replace Proposition   \ref{LemExpectq} (for the supermartingale property) with Proposition \ref{LemExpectq_2}; Corollary \ref{prop1} with Corollary \ref{prop1_again}; Proposition \ref{LemExpectq}b) with Proposition \ref{LemExpectq_2}b). We refer the reader to the proof of Proposition \ref{trans_prob_prop}.
%Lemma \ref{recurrence_prob_lemma} and Proposition \ref{LemExpectq}, for the proofs of Lemma \ref{recurrence_prob_lemma_2} and Proposition \ref{LemExpectq_2}.

\subsection{Rate of Convergence and Regret Bound.}
\label{app:regret}

Much of the remainder of the proof of Theorem \ref{2nd_theorem} is identical to the proof of Theorem \ref{main_theorem}. The final part applies Lemma \ref{last_lemma} (given below) in place of Lemma \ref{LemABC}, and Proposition \ref{LemExpectq_2}c) in place of Proposition \ref{LemExpectq}c). This obtains the modified regret bound.

\begin{lemma}\label{last_lemma}
	For $\theta>0$,
	\[
	\sum_{t=\lceil e/\theta \rceil+1}^T
	\frac{\log \theta t}{\theta t}
	\leq 
	\frac{1}{2\theta}
	(\log \theta T)^2\, .
	\]
\end{lemma}
\Beginproof
	The function $z \mapsto z^{-1}\log z $ is maximized at $z=e$ and is decreasing thereafter. For this reason
	\begin{align*}
	\sum_{t=\lceil e/\theta \rceil+1}^T
	\frac{\log \theta t}{\theta t}
	&
	\leq 
	\int_{e/\theta}^T
	\frac{1}{\theta t}\log (\theta t)
	dt
	=
	\frac{1}{\theta}
	\int_{e}^{\theta T}
	\frac{1}{t} \log t
	dt
	\\ 
	&
	=
	\frac{1}{\theta}
	\left[
	\frac{1}{2}
	(\log t)^2
	\right]^{\theta T}_{e}
	=
	\frac{1}{2\theta} 
	(\log \theta T)^2
	-
	\frac{1}{2\theta}\, .
	\end{align*}
	
\Endproof
%\beginproof
%a
%\endproof 

\proof{Proof of Theorem \ref{2nd_theorem}.}
	Note that by Proposition \ref{trans_prob_prop_2}c), we have that
	\[
	p_{a^\star}(t) = 1- q_{a^\star}(t) \xrightarrow[t\rightarrow\infty]{} 1.
	\]
	By the identical argument applied in Theorem \ref{main_theorem} we have that
	\[
	\mathcal R\! g(T)
	\leq 
	Q
	+
	\sum_{s=0}^{T-1} 
	\mathbb E \big[ 
	\hat q(s) 
	\big]\, .
	\]
	Applying Proposition \ref{LemExpectq_2} 
	and Lemma \ref{last_lemma} 
	\begin{align*}
	\sum_{s=0}^{T-1} 
	\mathbb E \big[ 
	\hat q(s) 
	\big]
	&
	\leq 
	\Big\lceil \frac{e}{\beta \Delta} \Big\rceil 
	+
	\sum_{s=\lceil \frac{e}{\beta \Delta} \rceil +1 }^{T} 
	\mathbb E \big[ 
	\hat q(s) 
	\big]	
	\\	
	&
	\leq 
	\Big\lceil \frac{e}{\beta \Delta} \Big\rceil 
	+
	\sum_{s=\lceil \frac{e}{\beta \Delta} \rceil +1 }^{T} 	
	\frac{N}{s \beta \Delta} \log (s \beta \Delta)
	\\
	&
	\leq 
	\Big\lceil \frac{e}{\beta \Delta} \Big\rceil 
	+
	\frac{N}{2\beta\Delta}
	(\log \beta\Delta T)^2\, .
	\end{align*}
	Combining this with the above inequality gives 
	\begin{equation*}
	\mathcal R\! g(T)
	\leq 
	\frac{N}{2\beta\Delta}
	(\log \beta\Delta T)^2
	+
	Q
	+
	\Big\lceil \frac{e}{\beta \Delta} \Big\rceil 
	\end{equation*}
	as required.
\endproof



